Dynamics of Hot QCD Matter -- Current Status and Developments

The discovery and characterization of hot and dense QCD matter, known as Quark Gluon Plasma (QGP), remains the most international collaborative effort and synergy between theorists and experimentalists in modern nuclear physics to date. The experimentalists around the world not only collect an unprecedented amount of data in heavy-ion collisions, at Relativistic Heavy Ion Collider (RHIC), at Brookhaven National Laboratory (BNL) in New York, USA, and the Large Hadron Collider (LHC), at CERN in Geneva, Switzerland but also analyze these data to unravel the mystery of this new phase of matter that filled a few microseconds old universe, just after the Big Bang. In the meantime, advancements in theoretical works and computing capability extend our wisdom about the hot-dense QCD matter and its dynamics through mathematical equations. The exchange of ideas between experimentalists and theoreticians is crucial for the progress of our knowledge. The motivation of this first conference named "HOT QCD Matter 2022" is to bring the community together to have a discourse on this topic. In this article, there are 36 sections discussing various topics in the field of relativistic heavy-ion collisions and related phenomena that cover a snapshot of the current experimental observations and theoretical progress. This article begins with the theoretical overview of relativistic spin-hydrodynamics in the presence of the external magnetic field, followed by the Lattice QCD results on heavy quarks in QGP, and finally, it ends with an overview of experiment results.

==> Debarshi/bib.tex <==
%%%%%%%%Lokesh begins%%%%%%%%

\bibitem{sokov:IJMPA24'2009} V. V. Sokov, A. Y. Illarionov, and V. D. Toneev, {\it International Journal of Modern Physics A} {\bf 24} (2009) 5925.

\bibitem{tuchin:PRC82'2010} K. Tuchin, {\it Phys. Rev. C} {\bf 82}, 3 (2010).

\bibitem{kharzeev:NPA803'2008} D. E. Kharzeev, L. D. McLerran, and H. J. Warringa, {\it Nuclear Physics A} {\bf 803}, 227 (2008).

\bibitem{fukushima:PRL120'2018}K. Fukushima and Y. Hidaka, {\it Phys. Rev. Lett.} {\bf 120}, 162301 (2018).

\bibitem{Schenke:PRL108'2012} B. Schenke, P. Tribedy, and R. Venugopalan, {\it Phys. Rev. Lett.} {\bf 108}, 252301 (2012).

\bibitem{Karmakar:EPJC79'2019}B. Karmakar, A. Bandyopadhyay, N. Haque, M. G. Mustafa, {\it The European Physical Journal C} {\bf 79}, 658  (2019).

\bibitem{Das:PRD97'2018} A. Das, A. Bandyopadhyay, P. K. Roy, and M. G.
Mustafa, {\it Phys. Rev. D} {\bf 97}, 034024 (2018).

\bibitem{Pushpa:PRD97'2022}P. Panday and B. K. Patra, {\it Phys. Rev. D} {\bf 105}, 116009  (2022).

\bibitem{Hosoya:NPB250'1985}A. Hosoya and K. Kajantie, {\it Nuclear Physics B} {\bf 250}, 666  (1985).

\bibitem{Callen} H. B. Callen, {\it Thermodynamics and an Introduction to
	Thermostatistics}, 2nd ed. (Wiley, New York, 1991).

\bibitem{Feng:PRD96'2017}B. Feng, {\it Phys. Rev. D} {\bf 96}, 036009  (2017).



%\bibitem{Ayala:PRD98'2018}A. Ayala, C. A. Dominguez, S. Hernandez-Ortiz, L. A.
%Hernandez, M. Loewe, D. M. Paret, and R. Zamora, {\it Phys. Rev. D} {\bf 98}, 031501  (2018).











 



%%%%%%%%Lokesh ends%%%%%%%%










==> Samapan/samapan2.tex <==
\title{Relativistic Dissipative Spin-hydrodynamics and spin-magnetohydrodynamics %\footnote{For the title, try not to use more than 3 lines. Typeset the title in 10 pt Times roman, uppercase and boldface.}
}

\author{Samapan Bhadury and Amaresh Jaiswal}



\begin{abstract}
We write semi-classical kinetic equations for a relativistic fluid of spin-\nicefrac{1}{2} particles within the relaxation time approximation, with and without magnetic field. Building on these, we then go on to formulate the theory of relativistic hydrodynamics in both cases. Consequently, we obtain the theories of relativistic dissipative spin-hydrodynamics and spin-magnetohydrodynamics. While in the former case, we find, for the first time, the dissipation mechanism of spin degrees of freedom, in the latter case, we note effects analogous to Einstein-de Haas and Barnett effects at the dissipation level.
\end{abstract}

\keywords{spin-polarization; relativistic hydrodynamics; magnetic field.}

\ccode{PACS numbers: 25.75.Nq, 25.75.-q, 05.20.Dd, 52.30.Cv, 52.65.Kj}




\section{Introduction}%General Appearance}

In the ultra-relativistic non-central heavy-ion collisions at the collider facilities such as Relativistic Heavy-Ion Collider (RHIC) and Large Hadron Collider (LHC), a large angular momentum \cite{Becattini:2007sr} as well as a large magnetic field \cite{Tuchin:2013ie} are generated at the early stages of the evolution, which can couple with the intrinsic spin of the constituent particle via the processes similar to Einstein-de Haas and Barnett effects. It was predicted that such couplings lead to the spin polarization of the medium \cite{Liang:2004ph, Liang:2004xn}, which can be observed in particles emitted during freeze-out. This was latter confirmed experimentally \cite{STAR:2017ckg, STAR:2018gyt, STAR:2019erd, ALICE:2019aid, STAR:2020xbm, STAR:2021beb} giving a significant boost to the study of spin-polarization.

The hydrodynamic models assuming equilibrated spin degrees of freedom successfully explained these observations of global spin-polarization but failed to show similar success in the case of longitudinal spin-polarization \cite{Li:2017dan, ALICE:2019aid}. This indicated different possible origins of spin-polarization, which then led to the belief that the spin degrees of freedom in the transverse plane may not achieve equilibration at the time of freeze-out \cite{Bhadury:2020cop}, and consequently, we may require dissipative theories of hydrodynamics.

Hence, we formulated a theory of relativistic dissipative spin-hydrodynamics first without the influence of an external field and then in the presence of a magnetic field from the relativistic kinetic theory that is consistent with macroscopic conservation laws. In the latter case, we found it may be possible to observe effects similar to Einstein-de Haas and Barnett effects if the fluid is magnetizable in addition to being spin-polarizable.

% Contributions to {\it International Journal of Modern Physics E} are
% to be in English. Authors are encouraged to have their contribution
% checked for grammar. American spelling should be used. Abbreviations
% are allowed but should be spelt out in full when first used. Integers
% ten and below are to be spelt out. Italicize foreign language phrases
% (e.g.~Latin, French).

% The text is to be typeset in 10 pt roman, single spaced with
% baselineskip of 13~pt. Text area (including copyright block)
% is 8 inches high and 5 inches wide for the first page.  Text area
% (excluding running title) is 7.7 inches high and 5 inches wide for
% subsequent pages.  Final pagination and insertion of running titles
% will be done by the publisher.

\section{Relativistic Spin-hydrodynamics\label{RSH}}

The theory of hydrodynamics is built on the basis of conservation laws of the fluid under consideration. Such conservation laws lead to the equations of motion that govern the evolution dynamics of that specific fluid. Noting that the origin of spin-polarization is traced back to the rotation of the fluid, the relevant conservation laws for a spin-polarizable fluid are - (i) Particle/Baryon/Charge four-current, (ii) Stress-energy tensor, (iii) Angular momentum tensor. In this section, we will first provide the equations of motion of relativistic spin-polarized fluid of a single species, without a magnetic field and then with a magnetic field.

\subsection{Without magnetic field\label{RSH_B=0}}

The particle four-current of a dissipative relativistic fluid is given by,
%
\begin{align}
    N^\mu = n_0\, u^\mu + n^\mu, \label{RSH1:N^m_decomp}
\end{align}
%
where $n_0$ is the equilibrium particle number density, $n^\mu$ is particle diffusion current and $u^\mu$ is the fluid four-velocity. In writing Eq.~\eqref{RSH1:N^m_decomp} we have assumed the out-of-equilibrium number density is, $n = n_0$. This is one of the Landau matching conditions. Then the conservation law is,
%
\begin{align}
    \partial_\mu N^\mu = 0. \label{RSH1:del.N}
\end{align}
%
The next conservation law is for the stress-energy tensor of the fluid, which is given by,
%
\begin{align}
    T_{\rm f}^{\mu\nu} &= \epsilon_0 u^\mu u^\nu - \left( P + \Pi \right) \Delta^{\mu\nu} + \pi^{\mu\nu}, \label{RSH1:T^mn_decomp}
\end{align}
%
where $\epsilon_0$ is the equilibrium energy density, $P$ is the equilibrium pressure, $\Pi$ is the bulk viscous pressure, and $\pi^{\mu\nu}$ is the shear viscous pressure. As before, we have assumed in writing Eq.~\eqref{RSH1:T^mn_decomp} that the out-of equilibrium energy density is $\epsilon = \epsilon_0$, i.e., the other matching condition. Additionally, we also assumed the Landau frame definition for the fluid four-velocity, which satisfied the relation, $T^{\mu\nu} u_{\nu} = \epsilon u^{\mu}$. The associated conservation law is given by,
%
\begin{align}
    \partial_\mu T_{\rm f}^{\mu\nu} = 0. \label{RSH1:del.T}
\end{align}
%
The final relevant conservation law is the one for angular momentum tensor. This becomes important for rotating fluids and is given by,
%
\begin{align}
    \partial_\lambda J_{\rm f}^{\lambda,\mu\nu} = 0, \label{RSH1:del.J}
\end{align}
%
where $J_{\rm f}^{\lambda,\mu\nu}$ is the total angular momentum tensor of the fluid that consists of two parts, an orbital part ($L_{\rm f}^{\lambda,\mu\nu}$) and a spin part ($S^{\lambda,\mu\nu}$) i.e. $J_{\rm f}^{\lambda,\mu\nu} = L_{\rm f}^{\lambda,\mu\nu} + S^{\lambda,\mu\nu}$. As the orbital part is defined as the moment of the stress-energy tensor (i.e. $L_{\rm f}^{\lambda,\mu\nu} = x^\mu T_{\rm f}^{\lambda\nu} - x^\nu T_{\rm f}^{\lambda\mu}$), it does not carry any new information that was not already present in the stress-energy tensor. Therefore, the good conservation law to describe system is the one for spin tensor and for a symmetric tress-energy tensor, we have,
%
\begin{align}
    \partial_\lambda S^{\lambda,\mu\nu} = 0. \label{RSH1:del.S}
\end{align}
%
Thus, Eqs.~\eqref{RSH1:del.N}, \eqref{RSH1:del.T} and \eqref{RSH1:del.S} are the conservation laws satisfied by a relativistic spin-polarizable fluid in absence of any external field.

\subsection{ With magnetic field\label{RSH_B_neq_0}}

The next step is to consider the effect of the magnetic field. The conservation law for the particle four-current remains the same, and since we consider only a single species, the charge four-current of the fluid is simply $J^\alpha_{\rm f} = \mathfrak{q} N^\mu$ ($\mathfrak{q}$ being the particle's electric charge). Since it is the charge currents that generate the magnetic field, it is important to note that other charge currents may exist ( say, $J^\mu_{\rm ext}$). In fact, in the case of heavy-ion collisions, the charged current that produces the majority of the magnetic field is that of the spectator particles. The field strength tensor due to the total current, $J^\mu$ ($= J^{\mu}_{\rm f} + J^{\mu}_{\rm ext}$) is $F^{\mu\nu}$. While the conservation law for the particle four-current still holds true, the laws for energy and momentum (both linear and angular) for the fluid are no longer satisfied due to interaction with the produced field. Consequently, the fluid stress-energy tensor ($T^{\mu\nu}_{\rm f}$) and angular momentum tensor ($J^{\lambda,\mu\nu}_{\rm f}$) do not remain conserved. One should note that the conservation laws for the whole system are still satisfied \cite{Bhadury:2022qxd}. Hence for a spin-polarizable magnetizable fluid, we have,
%
\begin{align}
    %1
    \partial_\nu T^{\mu\nu}_{\rm f} &= F^{\mu}_{~\, \alpha} J^{\alpha}_{\rm f} + \frac{1}{2} \left( \partial^\mu F^{\alpha\beta} \right) M_{\alpha\beta}, \label{RSH2:del.T}\\
    %2
    \partial_\lambda J^{\lambda,\mu\nu}_{\rm f} &= -\tau^{\mu\nu}, \label{RSH2:del.J}
\end{align}
%
where $M^{\alpha\beta}$ is the magnetization tensor and $\tau^{\mu\nu}$ is the torque generated by the force term appearing on the R.H.S. of Eq.~\eqref{RSH2:del.T}. Owing to the definition of the orbital angular momentum, we can show the spin tensor is still conserved, and we get back Eq.~\eqref{RSH1:del.S}. Hence, the only relevant modification in conservation laws for the formulation of spin-magnetohydrodynamics as compared to field-free case is in Eq.~\eqref{RSH2:del.T}. Therefore, the equations of motion of relativistic spin-magnetohydrodynamics are give by Eqs.~\eqref{RSH1:del.N}, \eqref{RSH1:del.S} and \eqref{RSH2:del.T}. Next, we describe the kinetic theory formulation of spin hydrodynamics, with and without magnetic field.

\section{Relativistic Kinetic Theory\label{RKT}}

Spin, being a purely quantum mechanical effect, must be introduced in the kinetic theory via quantum field theory. Hence, our starting point is the Wigner function for spin-$\nicefrac{1}{2}$ particles and its Clifford-algebra decomposition \cite{Elze:1986hq, Elze:1986qd, Vasak:1987um, Weickgenannt:2019dks, Weickgenannt:2020aaf, Sheng:2021kfc},
%
\begin{align}
    \mathcal{W}(x,k) &= \frac{1}{4} \left[ \mathcal{F}(x,k) \!+\! i \gamma_5 \mathcal{P}(x,k) \!+\! \gamma^\mu {\cal V}_{\mu}(x,k) \!+\! \gamma_5 \gamma^\mu {\cal A}_{\mu}(x,k) \!+\! \Sigma^{\mu\nu} {\cal S}_{\mu \nu}(x,k) \right]\!, \label{RSH:wig_decomp}
\end{align}
%
where $x$ is the space-time coordinate, $k^\mu = (k^0, \textbf{k})$ denotes the particle momentum and, $\gamma^\mu$ are the Dirac gamma matrices with $\gamma^5 = i \gamma^0 \gamma^1 \gamma^2 \gamma^3$. It is possible to show that not all the coefficients of the right-hand side of Eq.~\eqref{RSH:wig_decomp} are totally independent. For the formulation of spin-hydrodynamics, it suffices to work with only two of the components, which in our case are, the scalar component ($\mathcal{F}$) and the axial component ($\mathcal{A}$). Their kinetic equations can be obtained from the Dirac equation to be given by,
%
\begin{align}
    k^\mu \partial_\mu {\cal F}(x,k) = C_{\cal F},
    \qquad
    k^\mu \partial_\mu \, {\cal A}^\nu(x,k) = C^\nu_{\cal A}, 
    \qquad
    k_\nu \,{\cal A}^\nu(x,k) = k_\nu C^\nu_{\cal A} = 0, \label{RSH:kineqAC1}
\end{align}
%
where $\mathcal{C}_{\mathcal{F}}$ and $\mathcal{C}_{\mathcal{A}}^\mu$ are the collision kernels. In the absence of an external field, following the approach as described in Ref.~\cite{Bhadury:2020puc}, we can obtain a Boltzmann-like equation of scalar phase-space distribution functions, $f^\pm(x,p,s)$ with an extended phase-space for particles and anti-particles under the relaxation time approximation as,
%
\begin{align}
    p^\mu \partial_\mu f^\pm(x,\textbf{p},s) = \left(u \cdot p\right) \frac{f^\pm_{\rm eq}(x,\textbf{p},s)-f^\pm(x,\textbf{p},s)}{\tau_{\rm eq}}, \label{RSH:Beq1}
\end{align}
%
where $\tau_{\rm eq}$ is the relaxation time. We can use this distribution function, $f(x,\textbf{p},s)$ to express the scalar and axial components of the Wigner function. The zeroth and first moment of Eq.~\eqref{RSH:Beq1} will result in the conservation laws of Eqs.~\eqref{RSH1:del.N} and \eqref{RSH1:del.T} and the spin moment will lead to Eq.~\eqref{RSH1:del.S} provided we use appropriate frame and matching conditions. One can easily check this by noting the definitions of the conserved currents from kinetic theory i.e.,
%
\begin{align}
    %1
    N^{\mu} &= \int dP dS p^\mu \left( f^+ - f^- \right), \label{RSH:N^m_defKT} \\
    %2
    T^{\mu\nu}_{\rm f} &= \int dP dS p^\mu p^\nu \left( f^+ + f^- \right), \label{RSH:T^mn_defKT} \\
    %3
    S^{\lambda,\mu\nu} &= \int dP dS s^{\mu\nu} \left( f^+ + f^- \right), \label{RSH:S^lmn_defKT}
\end{align}

where $dP \equiv  d^3p/[p^0 (2 \pi )^3]$ and $dS \equiv m/(\pi \mathfrak{s}) \,  d^4s \, \delta(s \cdot s + \mathfrak{s}^2) \, \delta(p \cdot s)$ are the momentum and spin integral measures respectively with $p^0$ being the zeroth component of the momentum four-vector and $\mathfrak{s}$ being the eigenvalue of the Casimir operator. In the presence of a magnetic field, however, we obtain a modified Boltzmann equation under RTA as,
%
\begin{align}
    \left( p^\alpha \dfrac{\partial }{\partial x^\alpha} + m\,\mathcal{F}^\alpha \dfrac{\partial }{\partial p^\alpha} %+ m\,\mathcal{S}^{\alpha\beta} \dfrac{\partial }{\partial s^{\alpha\beta}}
    \right) f^\pm &= - \left(u\cdot p\right) \frac{\left(f^\pm - f^\pm_{\rm eq}\right)}{\tau_{\rm eq}}\,,\label{RSH:Beq2}
\end{align}
%
where the force term is given by,
%
\begin{align}
    %1
    \mathcal{F}^\alpha &= \frac{d p^\alpha}{d \tau} = \frac{\mathfrak{q}}{m}\,  F^{\alpha\beta} p_\beta + \frac{1}{2} \left( \partial^\alpha F^{\beta\gamma} \right) m_{\beta\gamma}, \label{RSH:Beq_Force}
\end{align}
%
with $m^{\alpha\beta}$ being the magnetic dipole moment that is related to the internal angular momentum, $s^{\alpha\beta}$ as, $m^{\alpha\beta} = \chi s^{\alpha\beta}$. The quantity, $\chi$ is analogous to the gyromagnetic ratio. We can define the magnetization tensor, $M^{\alpha\beta}$ using this $m^{\alpha\beta}$ as,
%
\begin{align}
    M^{\alpha\beta} = m \int dP dS m^{\alpha\beta} \left( f^+ + f^- \right), \label{RSH:M_def}
\end{align}
%
where $m$ is the mass of the particle. It should be noted that in Eq.~\eqref{RSH:Beq2} we have left out one term that we call the `pure torque' term (associated to $d\mathcal{S}^{\alpha\beta}/d\tau$). A derivation of spin-magnetohydrodynamics with this term will be provided in some other publications. It is straightforward to recover Eq.~\eqref{RSH:Beq1} from Eq.~\eqref{RSH:Beq2} by setting $F^{\alpha\beta} \to 0$. We can arrive at the macroscopic conservation laws for spin-magnetohydrodynamics by starting from Eq.~\eqref{RSH:Beq2} and taking the zeroth, first and spin moments i.e. Eqs.~\eqref{RSH1:del.N}, \eqref{RSH2:del.T} and \eqref{RSH1:del.S}.


\section{Transport Coefficients\label{TC}}

We can now solve the Eqs.~\eqref{RSH:Beq1} and \eqref{RSH:Beq2} to obtain the non-equilibrium correction to the phase-space distribution functions and use them to get the dissipative currents. For this purpose, we consider a Chapman-Enskog like iterative expansion, where the out-of-equilibrium phase-space distribution function can be expressed as a sum of the equilibrium part ($f^\pm_{\rm eq}$) and the non-equilibrium correction part ($\delta f^\pm_{\rm eq}$) i.e.,
%
\begin{align}
    f^\pm (x,\textbf{p},s) = f_{\rm eq}^\pm (x,\textbf{p},s) + \delta f^\pm (x,\textbf{p},s). \label{RSH:CE_f}
\end{align}
%
We can use Eq.~\eqref{RSH:CE_f} in Eqs.~\eqref{RSH:Beq1} and \eqref{RSH:Beq2} to obtain the expressions of $\delta f^\pm (x,\textbf{p},s)$ in both cases of with and without magnetic field.

In the field-free case, we find the dissipative corrections to the currents, $N^\mu$ and $T^{\mu\nu}$ remain unaffected by the spin-polarization. However, we obtained the dissipation mechanism of the spin degrees of freedom for the first time to be given by \cite{Bhadury:2020puc},
%
\begin{align}
    \delta S^{\lambda,\mu\nu} &= \tau_{\rm eq} \Big[ B^{\lambda,\mu\nu}_{\Pi}\, \theta + B^{\kappa\lambda,\mu\nu}_{n}\, (\nabla_\kappa \xi) + B^{\alpha\kappa\lambda,\mu\nu}_{\pi}\, \sigma_{\alpha\kappa} + B^{\kappa\lambda\alpha\beta,\mu\nu}_{\Sigma}\, (\nabla_\kappa \omega_{\beta\alpha}) \Big]. \label{RSH:deltaS}
\end{align}
%
where, $\theta = \partial\cdot u$ is the scalar expansion, $\sigma^{\mu\nu} = \Delta^{\mu\nu}_{\alpha\beta} \partial^\alpha u^\beta$ is the shear stress tensor and, $\nabla^\alpha \xi$ and $\nabla^\alpha \omega^{\mu\nu}$ are the particle and spin diffusion respectively. Here we have defined the spacelike derivative as, $\nabla^\mu \equiv \Delta^\mu_\alpha \partial^\alpha$, with $\Delta^{\mu\nu} = g^{\mu\nu} - u^\mu u^\nu$ being the projection operator orthogonal to the fluid four-velocity. We have defined another projection operator is defined as, $\Delta^{\mu\nu}_{\alpha\beta} = \left( \Delta^\mu_\alpha \Delta^\nu_\beta + \Delta^\mu_\beta \Delta^\nu_\alpha \right)/2 -  \Delta^{\mu\nu} \Delta_{\alpha\beta}/3$ that is symmetric and traceless in the indices $\mu,\nu$ and $\alpha,\beta$.

In the presence of magnetic field, the dissipative currents for the spin-polarizable and magnetizable relativistic fluid are given by \cite{Bhadury:2022qxd},
%
\begin{align}
    %1
    n^{\mu} &= \tau_{\mathrm{eq}} \Big[ \beta_{n\Pi}^{\langle\mu\rangle}\, \theta 
    + \beta_{na}^{\langle\mu\rangle\alpha} \dot{u}_{\alpha}
    + \beta_{nn}^{\langle\mu\rangle\alpha} \left( \nabla_\alpha\xi \right) 
    + \beta_{nF}^{\langle\mu\rangle\alpha\beta} \left( \nabla_{\alpha} B_{\beta} \right) \nonumber\\
    %
    &\qquad\quad+ \beta_{n\pi}^{\langle\mu\rangle\alpha\beta} \sigma_{\alpha\beta}
    + \beta_{n\Omega}^{\langle\mu\rangle\alpha\beta} \Omega_{\alpha\beta} 
    + \beta_{n\Sigma}^{\langle\mu\rangle\alpha\beta\gamma} \left( \nabla_\alpha \omega_{\beta\gamma} \right) \Big], \label{RSH2:n}\\
    %2
    \Pi &= \tau_{\mathrm{eq}} \Big[ \beta_{\Pi\Pi}\, \theta 
    + \beta_{\Pi a}^{\alpha} \dot{u}_{\alpha} 
    + \beta_{\Pi n}^{\alpha} \left( \nabla_\alpha\xi \right) 
    + \beta_{\Pi F}^{\alpha\beta} \left( \nabla_{\alpha} B_{\beta} \right) 
    + \beta_{\Pi\pi}^{\alpha\beta} \sigma_{\alpha\beta} 
    + \beta_{\Pi\Omega}^{\alpha\beta} \Omega_{\alpha\beta} \nonumber\\
    %
    &\qquad\quad+ \beta_{\Pi\Sigma}^{\alpha\beta\gamma} \left( \nabla_\alpha \omega_{\beta\gamma} \right) \Big], \label{RSH2:Pi}\\
    %3
    \pi^{\mu\nu} &= \tau_{\mathrm{eq}} \Big[ \beta_{\pi\Pi}^{\langle\mu\nu\rangle} \theta 
    \!+ \beta_{\pi a}^{\langle\mu\nu\rangle\alpha} \dot{u}_{\alpha} 
    \!+ \beta_{\pi n}^{\langle\mu\nu\rangle\alpha}\! \left(\! \nabla_\alpha\xi \right)
    \!+\! \beta_{\pi F}^{\langle\mu\nu\rangle\alpha\beta}\! \left(\! \nabla_{\alpha} B_{\beta}\! \right) 
    \!+\! \beta_{\pi\pi}^{\langle\mu\nu\rangle\alpha\beta} \sigma_{\alpha\beta} \nonumber\\
    %
    &\qquad\quad+ \beta_{\pi\Omega}^{\langle\mu\nu\rangle\alpha\beta} \Omega_{\alpha\beta}
    \!+\! \beta_{\pi\Sigma}^{\langle\mu\nu\rangle\alpha\beta\gamma}\! \left(\! \nabla_\alpha \omega_{\beta\gamma} \right) \Big]\!, \label{RSH2:pi}\\
    %4
    \delta S^{\lambda,\mu\nu} &= \tau_{\mathrm{eq}}\, \Big[ B_{\Pi}^{\lambda,[\mu\nu]}\, \theta 
    + B_{a}^{\lambda,[\mu\nu]\alpha} \dot{u}_{\alpha} 
    + B_{n}^{\lambda,[\mu\nu]\alpha} \!\left( \nabla_\alpha \xi \right) 
    + B_{F}^{\lambda,[\mu\nu]\alpha\beta}\! \left( \nabla_{\alpha} B_{\beta} \right) \nonumber\\
    %
    &\qquad\quad+ B_{\pi}^{\lambda,[\mu\nu]\alpha\beta} \sigma_{\alpha\beta} 
    + B_{\Omega}^{\lambda,[\mu\nu]\alpha\beta} \Omega_{\alpha\beta} + B_{\Sigma}^{\lambda,[\mu\nu]\alpha\beta\gamma}\! \left( \nabla_\alpha \omega_{\beta\gamma} \right) \Big], \label{RSH2:delS}
\end{align}
%
where, $\Dot{u}^\mu \equiv \left(u\cdot\partial\right) u^\mu$ is the acceleration four-vector, $\Omega_{\alpha\beta} = \left(\nabla_\alpha u_\beta - \nabla_\beta u_\alpha\right)/2$ is the vorticity tensor and, $B^\alpha$ is the magnetic four-vector that is related to the field strength tensor as, $F^{\mu\nu} = \epsilon^{\mu\nu\alpha\beta} u_\alpha B_\beta$. In Eqs.~\eqref{RSH:deltaS}-\eqref{RSH2:delS} the transport coefficients are denoted by $\beta_{i}$'s and $B_i$'s.

\section{Summary and Conclusion\label{S&C}}

In this work, we demonstrated how to formulate the relativistic dissipative hydrodynamics for spin-polarizable particles with and without magnetic field starting from the kinetic theory. First, we obtained the dissipation mechanism of the spin degrees of freedom of a relativistic fluid in absence of any magnetic field for the first time and found it to depend on multiple hydrodynamic gradients. Next, we extended the framework to study the effect of magnetic field on a spin-polarizable relativistic fluid at the dissipation level. We found that it is necessary to consider the system to be magnetizable if we want to observe the coupling between spin and magnetic field. In this case, we found that all the dissipative currents depend on multiple hydrodynamic gradients, showing resemblance to the Einstein-de Haas and Barnett effects for the first time.

% Major headings should be typeset in boldface with the first
% letter of important words capitalized.

% \subsection{Sub-headings}

% Sub-headings should be typeset in boldface italic and capitalize
% the first letter of the first word only. Section number to be in
% boldface roman.

% \subsubsection{Sub-subheadings}

% Typeset sub-subheadings in medium face italic and capitalize the
% first letter of the first word only. Section numbers to be in
% roman.

% \subsection{Numbering and spacing}

% Sections, sub-sections and sub-subsections are numbered in
% Arabic.  Use double spacing before all section headings, and
% single spacing after section headings. Flush left all paragraphs
% that follow after section headings.

% \subsection{Lists of items}

% Lists may be laid out with each item marked by a dot:
% \begin{itemlist}
% 	\item item one,
% 	\item item two.
% \end{itemlist}
% Items may also be numbered in lowercase roman numerals:
% \begin{romanlist}[(ii)]
% 	\item item one
% 	\item item two
% 	\begin{romanlist}[(b)]
% 		\item Lists within lists can be numbered with lowercase roman letters,
% 		\item second item.
% 	\end{romanlist}
% \end{romanlist}

% \section{Equations}

% Displayed equations should be numbered consecutively in each
% section, with the number set flush right and enclosed in
% parentheses
% \begin{equation}
% 	\mu(n, t) = {\sum^\infty_{i=1} 1(d_i < t,
% 		N(d_i)=n)}{\int^t_{\sigma=0} 1(N(\sigma) = n)d\sigma}\,. \label{one}
% \end{equation}

% Equations should be referred to in abbreviated form,
% e.g.~``Eq.~(\ref{one})'' or ``(2)''. In multiple-line
% equations, the number should be given on the last line.

% Displayed equations are to be centered on the page width.
% Standard English letters like x are to appear as $x$
% (italicized) in the text if they are used as mathematical
% symbols. Punctuation marks are used at the end of equations as
% if they appeared directly in the text.



% \section{Tables}

% Tables should be inserted in the text as close to the point of
% reference as possible. Some space should be left above and below
% the table.

% Tables should be numbered sequentially in the text in Arabic
% numerals. Captions are to be centralized above the tables.
% Typeset tables and captions in 8~pt Times roman with
% baselineskip of 10~pt.

% \begin{table}[pt]
% 	\tbl{Comparison of acoustic for frequencies for piston-cylinder problem.}
% 	{\begin{tabular}{@{}cccc@{}} \toprule
% 			Piston mass & Analytical frequency & TRIA6-$S_1$ model &
% 			\% Error \\
% 			& (Rad/s) & (Rad/s) \\ \colrule
% 			1.0\hphantom{00} & \hphantom{0}281.0 & \hphantom{0}280.81 & 0.07 \\
% 			0.1\hphantom{00} & \hphantom{0}876.0 & \hphantom{0}875.74 & 0.03 \\
% 			0.01\hphantom{0} & 2441.0 & 2441.0\hphantom{0} & 0.0\hphantom{0} \\
% 			0.001 & 4130.0 & 4129.3\hphantom{0} & 0.16\\ \botrule
% 	\end{tabular}}
% 	\begin{tabnote}
% 		Table notes
% 	\end{tabnote}
% 	\begin{tabfootnote}
% 		\tabmark{a} Table footnote A\\
% 		\tabmark{b} Table footnote B
% 	\end{tabfootnote}
% \end{table}

% If tables need to extend over to a second page, the continuation
% of the table should be preceded by a caption,
% e.g.~``{\it Table 2.} $(${\it Continued}$)$''


% \noindent
% \begin{equation}
% 	\mu(n, t) = {\sum^\infty_{i=1} 1(d_i < t, N(d_i)
% 		= n)}{\int^t_{\sigma=0} 1(N(\sigma) = n)d\sigma}\,. \label{a1}
% \end{equation}

% \section{Footnotes}

% Footnotes should be numbered sequentially in superscript
% lowercase roman letters.\footnote{Footnotes should be
% 	typeset in 8~pt Times roman at the bottom of the page.}



% \section{Introduction}
% The ALICE experiment at the Large Hadron Collider has collected a large
% amount of data for various systems and energies\cite{1,2,3}.
% It is possible to study the  
% multiplicity dependence of various observables \cite{4}. 
% Many interesting observations in Refs.~\citen{2,3,4} have come out of ALICE
% by comparing results from of small systems pp and p-Pb with large systems Pb-Pb
% and Xe-Xe. 

% \subsection{Collectivity}\label{Sec:collect}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}%[h]
% 	\begin{center}
% 		%\rotatebox{0}{\resizebox{\columnwidth}{!}{
% 				%        \includegraphics{Figures/2019-06-06-LFmeanPt_logx_0.pdf}}}
% 		%\includegraphics[width =
% 		%12cm]{Figures/2019-06-06-LFmeanPt_logx_0.pdf}
% 		\includegraphics[width=9cm]{prabhakar/VsEtaCent2.pdf}
% 		\caption{Charged particle pseudorapidity density for various centrality
% 			classes over a broad range of $\eta$ in Xe-Xe collisions at $\sqrt{s_{NN}} =$ 5.44 TeV~\cite{8}. 
% 		}\label{Fig:eta}
% 	\end{center}
% \end{figure}

% \subsection{Summary}
% %
% In summary, we have presented a selected recent results on particle
% production from ALICE. The latest results on charged particle
% multiplicity confirm the violation of scaling of number of participant
% nucleons. 



% \section*{Acknowledgements}

% This section should come before the References. Funding
% information may also be included here.

% \appendix

% \section{Appendices}

% Appendices should be used only when absolutely necessary. They
% should come after the References. If there is more than one
% appendix, number them alphabetically. Number displayed equations
% occurring in the Appendix in this way, e.g.~(\ref{a1}), (A.2),
% etc.

==> Subash/definition.tex <==
%
% custom definitions
%
\newcommand {\roots}    {\ensuremath{\sqrt{s}}}
\newcommand {\sqrtsNN}  {\ensuremath{\sqrt{s_{_{\text{NN}}}}}}
\providecommand{\KS}{\ensuremath{\mathrm{K^0_S}}}
\providecommand{\LM}{\ensuremath{\Lambda}}
\providecommand{\ALM}{\ensuremath{\overline{\Lambda}}}
\providecommand{\KSKS}{\ensuremath{\mathrm{K^{0}_{S}K^{0}_{S}}}}
\providecommand{\LLALAL}{\ensuremath{\Lambda\Lambda\oplus\overline{\Lambda}\overline{\Lambda}}}
\providecommand{\LAL}{\ensuremath{\Lambda\overline{\Lambda}}}
\providecommand{\ALMALM}{\ensuremath{\overline{\Lambda}\overline{\Lambda}}}
\providecommand{\LMLM}{\ensuremath{\Lambda\Lambda}}
\providecommand{\LKS}{\ensuremath{\Lambda\mathrm{K^0_S}}}
\providecommand{\ALKS}{\ensuremath{\overline{\Lambda}\mathrm{K^0_S}}}
\providecommand{\LALKS}{\ensuremath{\Lambda\mathrm{K^0_S}\oplus\overline{\Lambda}\mathrm{K^0_S}}}
\providecommand{\VZ}{\ensuremath{\textrm{V}^{0}}}
\providecommand{\roots}{\ensuremath{\sqrt{s}}}

==> Sudipan/sudipanold.tex <==
 \section{Spatial Diffusion of Heavy Quarks in Magnetic Field}
 \author{Sudipan De}	
 
 \bigskip
 
\begin{abstract}
Heavy quarks are one of the most important tools to probe Quark Gluon Plasma (QGP) due to their large masses, which are significantly higher than the quantum chromodynamics (QCD) energy scale and the temperature at which QGP is created. In the recent years, off-central heavy ion collisions have gained a lot of attention owing to the possibility of the creation of strong magnetic fields of the order of 10$^{18}$ Gauss at the Relativistic Heavy-Ion collider (RHIC) and $\sim$10$^{19}$ Gauss at the Large Hadron Collider (LHC). In presence of this strong magnetic field, spatial diffusion coefficient of heavy quark splits into two components viz. transverse and longitudinal components. In the present work, we have estimated spatial diffusion of heavy quarks as a function of magnetic field and temperature.

\end{abstract}

\keywords{Kinetic theory; magnetic field; heavy flavour.}

\ccode{PACS numbers:}

\subsection{Introduction}

During the collisions of two nuclei at relativistic energies it is expected to form a hot and dense state of matter known as Quark Gluon Plasma (QGP) which is governed by light quarks and gluons~\cite{Shuryak:2004cy}. Heavy quarks, namely charm ($c$) and bottom $(b)$ quarks are considered one of the fine probes of quark gluon plasma (QGP). Due to the fact that their masses $(M)$ are significantly larger than the QCD energy scale ($\Lambda_\text{QCD}$) and the temperature ($T$) at which QGP is created i.e $ M >> \Lambda_\text{QCD}, T$. Unlike the light quarks they do not thermalize quickly and witness the entire evolution of the fireball. Currently, it is admitted that a very strong magnetic field is created at very early stage of heavy-ion collisions~\cite{Skokov:2009qp,Bzdak:2011yy}. The estimated values of the intensity of the strong magnetic field created at RHIC and LHC is of the order of $10^{18}$ to $10^{19}$ Gauss~\cite{Tuchin:2013ie}. The effects of such a strong magnetic field is discussed in different cases such as jet quenching coefficient $\hat{q}$~\cite{Banerjee:2021sjm}, elliptic flow~\cite{Das:2016cwd}, chiral magnetic effect~\cite{Kharzeev:2007jp} etc. The effect has also been studied to diffusion coefficients of charm quarks~\cite{Fukushima:2015wck,Finazzo:2016mhm}. As heavy quarks produced early in the heavy-ion collisions their dynamics can be affected by such strong magnetic field. 
In this article we aim to study the longitudinal and transverse components of diffusion coefficients of heavy quarks in a QGP medium in the presence of a background magnetic field $\vec{B}$ in $z$-direction.  

\subsection{Formulation}
Let us consider a background magnetic field $\vec{B} = B~\hat{k}$ pointing in the $z$-direction which magnetizes a relativistic fluid. In presence of magnetic field anisotropic properties of the fluid is considered which leads to multi-component structure of the electrical conductivity tensor such as, $\sigma_{xx}$, $\sigma_{xy} = -\sigma_{yx}$ and $\sigma_{zz}$. In this article we obtained diffusion coefficient in two different approaches, one is classical based Relaxation Time Approximation (RTA) method and another is Quantum Mechanical (QM) approximation. According to Einstein's relation the spatial diffusion coefficient $(D)$ can be expressed as a ratio of electrical conductivity $(\sigma)$ and susceptibility $(\chi)$ of the medium. These become anisotropic in the presence of magnetic field thus taking a $3\times 3$ matrix structure given by  
\bea
D_{ij} = \frac{\sigma_{ij}}{\chi},~~~i,j = x,y,z
\eea 
where $D_{ij}$ is the spatial diffusion matrix, $\sigma_{ij}$ is the electrical conductivity matrix, and  $\chi$ is the susceptibility. 
According to RTA approach we obtain
\bea
&&\sigma_{zz} = \sigma_\parallel = \frac{gq^2\beta}{3}\int\frac{d^3k}{(2\pi)^3}\frac{(k_z)^2}{\omega_k^2}\tau_cf\big[1-f\big]  \\
&&\sigma_{xx} = \sigma_{yy} = \sigma_\perp = \frac{gq^2\beta}{3}\int\frac{d^3k}{(2\pi)^3}\frac{(k_{x,y})^2}{\omega_k^2}\frac{\tau_c}{ 1 + \frac{\tau_c^2}{\tau_B^2}}f\big[1-f\big],
\label{eq:RTAsigmazz}
\eea
where, $f$ represents the distribution function such as,
\bea 
f = \begin{cases}
	\big[e^{\beta(\omega_k-\mu)} +1\big]^{-1},~{\rm~for~Fermions} \\
	\big[e^{\beta \omega_k} -1\big]^{-1},~{\rm~for~Bosons~~,}
\end{cases} 
\eea 
$\omega_k = \sqrt{\vec{k}^2 + m^2}$ is the energy with momentum $\vec{k}$ and mass $m$,  $\beta = T^{-1}$, where $T$ is the temperature, $\mu$ is the chemical potential, $q$ is the charge and $\tau_{c}$ is the relaxation time.
Here, $g$ is the degeneracy factor and $\tau_{B} = \frac{m}{q B}$ is the inverse of classical cyclotron frequency. $\sigma_{zz}$ (or $\sigma_\parallel$) is the parallel component of the electrical conductivity i.e. parallel to the magnetic field and $\sigma_{xx}$ (or $\sigma_\perp$) is the perpendicular component of the electrical conductivity. The absence of Landau quantization over energies in RTA expressions prompts us to call them as classical results. On the other hand, on applying Landau quantization of energies and quantizing the phase space part of the momentum integral we obtain

\bea
\chi_\text{QM} = \beta\sum_{n=0}^{\infty}(2-\delta_{n,0})\frac{qB}{2\pi}\int_{-\infty}^{+\infty}\frac{dk_z}{2\pi}~f(1-f).
\eea 



\bea
\sigma_\perp^\text{QM} &=& \frac{2q^2}{T}\sum_{n=0}^\infty (2-\delta_{n,0})\frac{qB}{2\pi}\int_{-\infty}^{+\infty}\frac{dk_z}{2\pi}\frac{lqB}{\omega_l^2}\tau^\perp f(1-f)
\label{ecqm:perp}\\
\sigma_\parallel^\text{QM} &=& \frac{2q^2}{T}\sum_{n=0}^\infty (2-\delta_{n,0})\frac{qB}{2\pi}\int_{-\infty}^{+\infty}\frac{dk_z}{2\pi}\frac{k_z^2}{\omega_l^2} \tau^\parallel f(1-f),
\label{ecqm:pll}
\eea 
where the superscript QM denotes quantum theoretical results, $\tau^\parallel = \tau_c$, $\tau^\perp = \frac{\tau_c}{1 + \frac{\tau_c^2}{\tau_B^2}}$, $\tau_c$ is the relaxation time.

\subsection{Results}

The left figure of the upper panel of Fig.~\ref{Fig:diffusion} shows the results of longitudinal diffusion as a function of temperature by plotting $2\pi T D_{zz}$ with $T$ which basically shows how the heavy quarks can diffusively travel in a direction parallel to the background magnetic field. In this figure the solid lines are for the isotropic case calculated via RTA formalism for $\tau_c = 6~fm$ and $eB$ = 0.2 and 0.4 GeV$^2$. The dotted lines are the results of $2\pi T D_{zz}$ for QM case where Landau quantization were employed, thus providing an expression of spatial diffusion as a sum over Landau levels. The increasing trend of diffusion coefficient with temperature can be attributed to the fact that an increase in kinetic energy contributes to an increase in diffusion along the direction parallel to magnetic field.
\begin{figure}[h]
	\begin{center}
		\includegraphics[width = 5cm]{Sudipan/pll-T-eps-converted-to.pdf}
		\includegraphics[width = 5cm]{Sudipan/pll-B-eps-converted-to.pdf}
		\includegraphics[width = 5cm]{Sudipan/perp-T-eps-converted-to.pdf}
		\includegraphics[width = 5cm]{Sudipan/perp-B-eps-converted-to.pdf}
		\caption{Upper panel: solid line shows the result from RTA calculation and dotted line shows results from QM approximation. Lower Panel: Black solid line represents the RTA result without magnetic field. Solid and dotted lines represent the results from RTA and QM respectively. Different colors represent the results at different magnetic fields as well as at different temperatures.
		}\label{Fig:diffusion}
	\end{center}
\end{figure}
The right figure of the upper panel of Fig.~\ref{Fig:diffusion} shows the results of longitudinal diffusion as a function of magnetic field by plotting $2\pi T D_{zz}$ with $eB$ at two different temperatures 0.2 GeV and 0.4 GeV for both RTA and QM formalisms. At low magnetic field the RTA and QM results coincide with each other whereas at high magnetic fields we see a clear deviation of QM results from RTA results which implies the universal behaviour of spatial diffusion at low magnetic field.  The longitudinal component of diffusion calculated via RTA formalism, does not depend on the magnetic field since along the direction of magnetic field the heavy quarks do not experience Lorentz force. Contrary to the RTA case, the QM results depend on the magnetic field. Here we see that for the QM case the diffusion increases with increasing magnetic field. To understand this we note that spatial diffusion is the ratio of electrical conductivity and static susceptibility. In the QM  approach the Landau level summation appears in the expression of $\sigma$ and $\chi$ due to which quantum effects come into play and thus we observe a deviation relative to RTA results. The left figure of the lower panel of Fig.~\ref{Fig:diffusion} shows the results of perpendicular component of spatial diffusion coefficient as a function of temperature for two different magnetic field strength, $eB$ = 0.2 GeV$^2$ and 0.4 GeV$^2$ along with the RTA results without presence of magnetic field. It is observed that in presence of strong magnetic field diffusion decreases. The right figure of the lower panel of Fig.~\ref{Fig:diffusion} shows the belabour of $D_{xx}$ with magnetic field for different values of temperatures. At low magnetic field the RTA and QM results coincide implying the universal nature of diffusion at low magnetic field whereas at high magnetic field they are different due to Landau level summation present in QM expressions.   

\subsection{Summary}
The spatial component of diffusion coefficient for heavy quarks was calculated in presence of strong background magnetic field using the well known Einstein relation. As diffusion coefficient becomes anisotropic in presence of magnetic field, both parallel and perpendicular components of diffusion coefficient were obtained. It is found that diffusion coefficient increases with increasing temperature both for parallel and perpendicular components. This behaviour can be attributed to the increase in kinetic energy of heavy quarks with increasing temperature. The difference between RTA and QM results is higher at higher magnetic field due to Landau level summation present in QM expression. Parallel component of diffusion coefficient is independent of magnetic field in case of RTA formulation contrary to the results obtained in QM formalism. Perpendicular component of diffusion coefficient decreases with increasing magnetic field both for RTA and QM. In summary, different belabour of parallel and perpendicular component of spatial diffusion coefficient of heavy quarks in presence of strong initial magnetic field may lead us to interesting directions in recent future. 

\subsection*{Acknowledgements}

Sudipan De and Sarthak Satapathy acknowledge financial support from the DST INSPIRE Faculty research grant (IFA18-PH220), India.

%\appendix

%\section{Appendices}




